REFUGE Challenge: A Unified Framework for Evaluating Automated Methods for Glaucoma Assessment from Fundus Photographs

Glaucoma is one of the leading causes of irreversible but preventable blindness in working age populations. Color fundus photography (CFP) is the most cost-effective imaging modality to screen for retinal disorders. However, its application to glaucoma has been limited to the computation of a few related biomarkers such as the vertical cup-to-disc ratio. Deep learning approaches, although widely applied for medical image analysis, have not been extensively used for glaucoma assessment due to the limited size of the available data sets. Furthermore, the lack of a standardize benchmark strategy makes difficult to compare existing methods in a uniform way. In order to overcome these issues we set up the Retinal Fundus Glaucoma Challenge, REFUGE (\url{https://refuge.grand-challenge.org}), held in conjunction with MICCAI 2018. The challenge consisted of two primary tasks, namely optic disc/cup segmentation and glaucoma classification. As part of REFUGE, we have publicly released a data set of 1200 fundus images with ground truth segmentations and clinical glaucoma labels, currently the largest existing one. We have also built an evaluation framework to ease and ensure fairness in the comparison of different models, encouraging the development of novel techniques in the field. 12 teams qualified and participated in the online challenge. This paper summarizes their methods and analyzes their corresponding results. In particular, we observed that two of the top-ranked teams outperformed two human experts in the glaucoma classification task. Furthermore, the segmentation results were in general consistent with the ground truth annotations, with complementary outcomes that can be further exploited by ensembling the results.

==> evaluated_methods.tex <==

\begin{table*}[t]  
\centering
\caption{Summary of main characteristics of the glaucoma classification methods evaluated in the on-site challenge, in alphabetical order using the teams names.}
\resizebox{\textwidth}{!}{
\begin{tabular}{C{1.8cm}|C{2cm}|C{2.8cm}|C{3cm}|C{6.5cm}|C{1.5cm}}
  \hline
  \textbf{Team} & \textbf{Inputs} & \textbf{Architectures} & \textbf{Training set} & \textbf{Methodology}  & \textbf{Post-processing} \\
  \hline
  AIML & Full image / ONH area & ResNet-50, -101, -152~\cite{he2016deep}, 38~\cite{wu2019wider} & REFUGE training set & Ensemble of glaucoma likelihoods from multiple networks fine-tuned from ImageNet & Ensemble by averaging \\ 
  \hline
  BUCT & ONH area, grayscale & Xception~\cite{chollet2017xception} & REFUGE training set & Training from scratch on grayscale images & None \\
  \hline
  CUHKMED & OD/OC segmentation & None & None & vCDR values computed from ellipses fitted to automated OD/OC segmentations & None \\
  \hline
  Cvblab & Full image & VGG19~\cite{simonyan2014very}, Inception V3~\cite{szegedy2016rethinking}, ResNet-50~\cite{he2016deep}, Xception~\cite{chollet2017xception} & REFUGE training set, DRISHTI-GS, HRF, ORIGA and RIM-ONE r3 & Ensemble of glaucoma likelihoods from multiple networks fine-tuned from ImageNet, classes in REFUGE training set balanced using SMOTE~\cite{chawla2002smote} & Ensemble by averaging \\
  \hline
  Mammoth & ONH area with CLAHE & ResNet-18~\cite{he2016deep} and CatGAN~\cite{wang2017catgan} & REFUGE training set (4-fold cross-validation) & Ensemble of ResNet models pre-trained from ImageNet and fine-tuned using REFUGE data and synthetic images generated with CatGAN & Ensemble by averaging \\
  \hline
  NightOwl & ONH area with/without exp. transform & Custom & REFUGE training set (10-fold cross-validation) & Ensemble of classification networks trained to predict glaucoma from features produced by the encoders of the segmentation networks & Ensemble by maximum \\
  \hline
  NKSG & Full image \JIOc{?} & SENet~\cite{Hu2018} & REFUGE training set (5-fold cross-validation) & SE-Net pretrained on images from Kaggle DR challenge~\cite{kaggledr} and fine-tuned on REFUGE data, best model from cross-validation taken for final prediction & None \\
  \hline
  SDSAIRC & Crop with ONH in upper-left corner & ResNet-50~\cite{he2016deep} & REFUGE training set & Logistic regression classifier trained with vCDR values from OD/OC segmentation and output of ResNet-50 model fine-tuned from ImageNet & None \\
  \hline
  SmileDeepDR & ONH area & DeepLabv3+~\cite{Chen2018} &  REFUGE training set & Adaptation of a segmentation network to predict a glaucoma likelihood & None \\
  \hline
  VRT & Full image with custom mask for attention & Custom~\cite{son2018classification} & Kaggle~\cite{kaggledr}, MESSIDOR~\cite{decenciere2014feedback} and IDRiD~\cite{porwal2018indian} & Attention guided model trained on public data sets of DR images, weakly labelled using pre-trained models for glaucoma classification, RNFL defects detection and segmentation of ONH pathological changes  & None \\
  \hline
  WinterFell & ONH area & ResNet-101, -152~\cite{he2016deep}, DensNet-169, -201~\cite{huang2017densely} & ORIGA & Ensemble of glaucoma likelihoods from multiple networks pre-trained on Image-Net and fine-tuned on ORIGA & Ensemble by mode, max. and min. \\
  \hline
\end{tabular}}
\label{table:submitted-glaucoma-classification} 
\end{table*}





==> previous_works_old.tex <==

\section{Previous works}
\label{sec:previous-works}

% In general, tasks such as glaucoma classification, optic disc/cup segmentation and fovea detection have been tackled using hand-crafted methods based on a combination of feature extraction techniques and either supervised or unsupervised machine learning classifiers~\cite{haleem2013automatic,almazroa2015optic,thakur2018survey}. More recently, convolutional neural networks (CNNs) have emerged as the state-of-the-art technique to apply for automated medical image analysis~\cite{litjens2017survey}. However, these approaches require large scale databases for training, which are costly and difficult to access publicly. As a consequence, their application to these tasks have been limited, and most of the developments in the field had to introduce solutions that somehow temper the effects of lacking enough training data. The REFUGE challenge aims to overcome this difficulty by introducing the largest available data set of CFP for glaucoma detection and assessment. Hence, although reviewing the extensive literature in the field is out of the scope of this paper, in this section we discuss some of these recent techniques and their key limitations. The interested reader could refer to \cite{haleem2013automatic,almazroa2015optic,thakur2018survey} for further information about other previous or alternative approaches. 


% \subsection{Optic disc and optic cup segmentation}
% \label{subsec:previous-methods-segmentation}

% Optic disc (OD) segmentation has been extensively studied in the past as it is relevant not only for glaucoma assessment but also in other applications such as characterizing the retinal vasculature~\cite{hemelings2018artery}, removing false positive detections of bright lesions~\cite{zhang2014exudate} or predicting the fovea position~\cite{meyer2018pixel}. When applied to AMD and DR cases, the major challenge is to be able to differentiate bright lesions from the OD intensities. In glaucomatous cases, however, the segmentation methods have to be robust against complex pathological ONH changes such as PPA (Fig.~\ref{fig:ppa}) or ONH hemorrhages~\cite{almazroa2015optic,thakur2018survey}. Furthermore, it is necessary to accurately segment the optic cup (OC), as both structures together are relevant to assess the ONH damage due to glaucoma, including the neuroretinal rim thinning. Segmenting the OC is a challenging task due to the high vessel density in the area. Moreover, the main feature to detect the OC edges accurately--the depth of the ONH--cannot be measured through a 2D projecting imaging modality such as CFP~\cite{miri2015multimodal}. Other features such as vessels bendings~\cite{joshi2011optic} or the image intensities~\cite{xu2014optic} have been studied in the past to approximate the ONH depth in CFP. In any case, all these factors turn the joint segmentation of the OD and the OC a significantly more challenging task that only identifying the OD boundaries.

% Two extensive reviews have been recently published summarizing the state of the art in joint OD/OC segmentation~\cite{almazroa2015optic,thakur2018survey}, with \cite{thakur2018survey} specifically focused on glaucoma assessment. In general, most of the approaches that are not based on deep learning use either custom image processing techniques such as feature enhancement and thresholding, or shape-prior guided algorithms such as level sets, active contours or active shape models. Other methods included the application of unsupervised clustering techniques, color analysis or hybrid combination of the above mentioned approaches~\cite{almazroa2015optic,thakur2018survey}. 

% Table~\ref{table:previous-segmentation-methods} lists the most recently published methods based on deep learning. It can be seen that most of them were trained and/or evaluated using different data sets and evaluation metrics, turning their comparison extremely difficult. Moreover, 

% To overcome the data limitation, the reviews approaches rely on the following strategies: (i) using patches instead of full size images for training, (ii) fine tunning deep CNNs trained on alternative databases, or (iii) applying U-shaped architectures. Patch-based segmentation algorithms intrinsically increase the size of the training sets by using patches rather than full images as training samples. However, this is done at the cost of reducing the field of view of the networks, affecting their ability to learn contextual features. As a consequence, these approaches usually require postprocessing techniques to remove spurious detection in wrong areas of the images. 

% Alternatively, the U-shaped architectures such as the U-Nets~\cite{ronneberger2015u} allow to learn accurate segmentation models from relatively small data sets using full images as inputs. 

% Transfer learning was also explored as an alternative to 

% In~\cite{zilly2015boosting}, a sampling strategy is introduced to learn a custom CNN architecture from a set of relevant points, and a boosting framework is used instead of the classical back-propagation based optimization to learn the CNN filters. \JIOc{check this}



% %The idea here is not only to summarize the current methods but also to show the variety of data sets and evaluation metrics used in each case. This will help us to underline the need of a common framework for evaluation.

% %\noindent \textcolor{red}{A description of current deep learning based approaches. There are only a few papers~\cite{fu2018joint,edupuganti2018automatic} that use really deep networks.\cite{edupuganti2018automatic} uses fine tunning from ImageNet weights to reduce the impact of the lack of data. Other papers use alternative strategies to deal with that. We should include a paragraph describing these strategies, to emphasize that most of the developments in deep learning for optic disc/cup segmentation were hampered before due to the lack of public available data.}


% \begin{table*}[t]  
% \centering
% \caption{Overview of recent deep learning based methods for joint optic disc (OD) and optic cup (OC) segmentation. IoU: intersection over union. NOR: non-overlap error, 1-IoU. MAE: mean absolute error of the CDR.}
% \begin{tabular}{C{2cm}|C{2.6cm}|C{1.2cm}|C{4cm}|C{1.5cm}|C{2.5cm}|C{1cm}}
%   \hline
%   \textbf{Reference} & \textbf{Preprocessing} & \textbf{Architecture} & \textbf{Methodology} & \textbf{Training set} & \textbf{Evaluation databases} & \textbf{Evaluation metrics} \\
% \hline
%   Lim \textit{et al.}, 2015~\cite{lim2015integrated} & Vessel inpainting, CLAHE on green and red channels, vessel bending enhancement & Patch-base LeNet & Modified LeNet architecture trained on patches to predict OD/OC probabilities, postprocessing  & \multicolumn{2}{C{4.5cm}|}{MESSIDOR, SEED-DB (private) (cross-validation)} & NOR, MAE \\ 
%   \hline
%   Zilly \textit{et al.}, 2015~\cite{zilly2015boosting} & Cropping + downsampling + L*a*b color space + Z-normalization & Custom CNN & Sampling strategy applied to identify relevant landmarks and boosting framework to learn the CNN filters & DRISHTI-GS1 (training set) & DRISHTI-GS1 (test set) & Dice, IoU \\ 
%   \hline
%   Sevastopolsky, 2017~\cite{sevastopolsky2017optic} & CLAHE + cropping using OD area & U-Net & U-Net with less and constant number of filters for each resolution & RIM-ONE v.3 & DRIONS-DB, RIM-ONE v.3, DRISHTI-GS1 & Dice, IoU \\ 
%   \hline
%   Al-Bander \textit{et al.}, 2018~\cite{al2018dense} & Detection of the horizontal insert points of the OD & FC-DenseNet  & U-shaped DenseNet for multiclass segmentation and postprocessing to remove spurious elements & ORIGA (random sample) & ORIGA, DRIONS-DB, DRISHTI-GS1, ONHSD, RIM-ONE & NOR, MAE \\
%   \hline
%   Edupuganti \textit{et al.}, 2018~\cite{edupuganti2018automatic} & None (RGB image) & FCN8s & Weighted loss (OD/OC pixels contribute 10 times more than background pixels) & DRISHTI-GS1 (training set) & DRISHTI-GS1 (test set) & IoU \\ 
%   \hline
%   Fu \textit{et al.}, 2018 \cite{fu2018joint} & OD detection + polar transformation & M-Net & Multiscale U-shape network trained on polar transformation of the input images & ORIGA (training set) & ORIGA, SCES & NOR, MAE\\
%   \hline
%   Sevastopolsky \textit{et al.}, 2018~\cite{sevastopolsky2018stack} & CLAHE & Stack-U-Net & Cascade: U-Net for initial segmentation and Res-U-Net for refinement & Not specified & DRIONS-DB, RIM-ONE v.3, DRISHTI-GS1, UCSF-DB (private) & Dice, IoU \\ 
%   \hline
%   Sun \textit{et al.}, 2018~\cite{sun2018localizing} & None (RGB image) & Faster R-CNN  & OD/OC detected with bounding boxes by the R-NN and transformed into ellipses  & ORIGA (training set) & ORIGA (test set) & NOR, MAE \\
%   \hline
% \end{tabular}
% \label{table:previous-segmentation-methods} 
% \end{table*}




% % \begin{table*}[t]  
% % \centering
% % \caption{Overview of recent deep learning based methods for joint optic disc (OD) and optic cup (OC) segmentation.}
% % \begin{tabular}{c|C{2cm}|C{5cm}|C{2cm}|C{2cm}}
% %   \hline
% %   \textbf{Reference} & \textbf{Architecture} & \textbf{Methodology} & \textbf{Evaluation database} & \textbf{Evaluation metrics} \\
% %   \hline
% %   Fu \textit{et al.} (2018) \cite{fu2018joint} & M-Net & U-shape network trained on polar transformation of the input images & ORIGA, SCES & Overlapping error (1 - Jaccard), CDR\\
% % %   \hline
% % %   \hline
% % %   Zilly \textit{et al.} (2017)~\cite{zilly2017glaucoma} & \multicolumn{3}{c|}{Deep learning} & DRISHTI-GS, RIM-ONE v3 & Pr, Re, Jaccard, Dice, BLE, CDR \\ % CDR: mean absolute error, standard deviation of the errors
% % %   \hline
% % %   Chakravarty \textit{et al.} (2017) \cite{chakravarty2017joint} & GMM and Conditional Random Field & Estimated depth map, color, radial gradients  & GMM + CRF & Private, DRISHTI-GS1 & Dice, BLE, Jaccard\\
% % %   \hline
% % %   Edupugant \textit{et al.} (2018) \cite{edupuganti2018automatic} & \multicolumn{3}{c|}{Deep learning} & DRISHTI-GS & Jaccard, Dice \\ 
% %   \hline
% % \end{tabular}
% % \label{table:previous-segmentation-methods} 
% % \end{table*}


% %   Raghavendra \textit{et al.} (2018) \cite{raghavendra2018deep} & 

% % existing approaches rely on the application of XXXXX. More recently, deep learning based solutions have been introduced~\cite{maninis2016deep} thanks to the availability of numerous data sets with OD segmentations (see Section~\ref{subsec:previous-databases}). The automated delineation of the OC, however, is significantly more challenging, as the depth of the ONH is the only feature that would allow to accurately segment the region but is not available in a 2D projective imaging modality such as fundus photography. Alternatively, the image intensities must be used, although the presence of vessel occlusions and the variations in the imaging conditions.

% % the depth of the ONH is the only characteristic that is

% % %Since its manual delineation is not as challenging as the 

% % % Main challenges of OD/OC segmentation
% % The simultaneous segmentation of the optic disc and the optic cup is challenging due to several reasons.
% % It is necessary to deal with the variations of intensities due to vessel occlusions, pathological changes around the optic disc (such as peripapillary atrophies) and variable imaging conditions.
% % Optic disc segmentation. In diseases such as DR and AMD, its detection is also difficulty by the presence of bright lesions such as exudates, whose intensities are similar to those on the OD. 

% % % Current literature is mostly focused on optic disc segmentation
% % Optic disc segmentation was better covered before. There are deep learning based systems that achieved remarkable performance in public databases~\cite{maninis2016deep}. There is a limited number of studies introducing techniques for optic cup segmentation, though. The density of vascular structures within the optic cup makes its segmentation particularly difficult~\cite{almazroa2015optic}.

% % % Generic analysis of previous approaches
% % An extensive analysis of previous methods for optic disc/cup segmentation was presented in~\cite{almazroa2015optic} and~\cite{thakur2018survey}. Most of previous approaches are based on: 
% % image preprocessing: vessel inpainting
% % feature extraction: wavelet, gradients, vessel kinking
% % segmentation based on thresholding: poor performance, early approaches
% % segmentation based on classification: superpixel classification using supervised methods, or unsupervised methods based on K means clustering.
% % segmentation based on active contours or level sets: natural way to impose ellipsoidal shape prior.

% % % More recent papers
% % % Sedai
% % Some methods are based on anatomical properties such as a high concentration of vessels or the bright intensities in the optic disc to detect the approximate location of the region of interest~\cite{sedai2016segmentation}
% % The segmentation is performed using an ensemble of shape regressors that try to link the visual appearance of the image with the approximate shape of the OD/OC structures. The outputs of the system are two contours that can be mapped into a binary segmentation mask. DRISHTI-GS training set with 5-fold cross-validation.~\cite{sedai2016segmentation}.
% % % Chakravarty
% % \cite{chakravarty2017joint}. Depth estimation, color features, radial gradients. GMM used to compute the unary potentials, pairwise term models the interaction between the optic disc/cup edges based in the depth. Several public available data sets INSPIRE, RIM-ONE v2, DRIONS-DB and MESSIDOR are used to evaluate its performance for optic disc detection. Results for optic disc/cup segmentation are evaluated in DRISHTI-GS1.



% % Papers that try to deal with the lack of enough data for applying deep learning.
% % In~\cite{zilly2017glaucoma} the authors trained a convolutional neural network for feature extraction, using a greedy approach instead of SGD optimization.
% % In~\cite{lim2015integrated} the authors proposed to adapt the input images by exagerating relevant visual features. To this end, the vessels are inpainted and the red and green bands from the RGB images are contrast equalized. Furthermore, the blue color channel is replaced by a vessel bending obtained by processing the skeletonized vessels. This allows to train a relatively shallow convolutional neural network with 3 convolutional and max-pooling layers and 2 fully convolutional layers, that classifies each pixel into OD, OC or background based on its $48\times48$ pixels neighborhood. A postprocessing stage is required to get a smooth representation of the OD and OC edges and to get rid of noisy responses. This might be a consequence of the shallow network applied for this task, which is not able to capture more relevant features to overcome this issue automatically.


% % To the best of our knowledge, the most recent approach for OD/OC segmentation based on deep learning is~\cite{sevastopolsky2018stack}. Two U-Net architectures~\cite{ronneberger2015u} architectures with ResNet~\cite{he2016deep} encoding blocks. \textcolor{red}{Check the paper.}
% % In~\cite{edupuganti2018automatic}, the authors introduce a fully connected CNN for optic disc/cup segmentation. The encoder is initialized with weights pre-learned from the ImageNet dataset. A weighted loss approach is used to leverage the disagreement between observers. The algorithm requires a postprocessing stage to remove spurious and noisy outputs.




% % BLE: Boundary Localization Error
% % CDR: Cup-to-disc ratio



% \subsection{Glaucoma detection}
% \label{subsec:previous-methods-glaucoma-detection}

% %Glaucoma detection consists in assigning a glaucoma likelihood or probability to an input image based in certain observed image features. Two extensive reviews have been introduced in the past covering most of the proposed automated methods to solve this task~\cite{haleem2013automatic, hagiwara2018computer}. 



% This section will include:
% \begin{itemize}
% \item Main challenges for glaucoma detection from fundus images. Subtle features that are barely visible in fundus images: PPA, retinal nerve fiber layer defects. We can use Figure~\ref{fig:glaucoma-detection-challenging} to ease the explanation.
% \item Citation to recent reviews in the field~\cite{haleem2013automatic,hagiwara2018computer} and a general description of the old methods. Most of them are based on hand crafted features such as textures, etc, that cannot be interpreted by physicians.
% \item A description of current deep learning based approaches, including transfer learning. Only a few. \cite{orlando2017convolutional} uses transfer learning on public database, using features from ImageNet and two architectures. \cite{li2018efficacy} used pure deep learning but for glaucoma optic neuropathy detection. 3 classes: no, suspect and certain. Uses 48.000 fundus images taken from a website, GT labels assigned by ophthalmologists based on image characteristics. Table~\ref{table:previous-glaucoma-detection-methods} will list them and some others, and show that most of them used different evaluation metrics/databases.
% \end{itemize}

% \begin{table*}[t]  
% \centering
% \caption{Overview of recent deep learning based methods for glaucoma detection from fundus photographs.}
% \begin{tabular}{c|C{2cm}|C{3cm}|C{3cm}|C{2cm}}
%   \hline
%   \textbf{Reference} & \textbf{Architecture} & \textbf{Methodology} & \textbf{Evaluation database} & \textbf{Evaluation metrics} \\
%   \hline
% %   Acharya \textit{et al.} (2017)~\cite{acharya2017novel} & Hand crafted & Texture (Texton and LCP) & kNN & Private & Acc, Pr, Se, Sp \\
% %   \hline
% %   Orlando \textit{et al.} (2017)~\cite{orlando2017convolutional} & Transfer learning & Deep learning features & L1/L2 logistic regression & DRISHTI-GS & AUC \\
%   \hline
% \end{tabular}
% \label{table:previous-glaucoma-detection-methods} 
% \end{table*}

% % LCP: Local configuration pattern



% \HFc{Shall we add the subsection for fovea localization?}


\subsection{Current public available data sets}
\label{subsec:previous-databases}

\begin{itemize}
\item List and description of current available data set. Short, we only want to include links to their websites, references to their original papers.
\item Table~\ref{table:database-comparison} summarizing their main characteristics. REFUGE is added so that we can show that these database is the largest one that has a tick for each category.
\item A discussion using the following important characteristics, that are covered by the REFUGE database.
\end{itemize}


%The availability of large scale, curated data sets of color fundus photographs for glaucoma detection and assessment is a key aspect to solve to promote the research in this field. So far, the previous initiatives has been limited in several aspects. We performed a systematic review of the literature in order to identify the existing databases of fundus pictures that provide annotations for glaucoma detection/classification, optic disc/cup segmentation and fovea localization. These three tasks are among the most important ones to be solved using automated algorithms. In particular, automated methods for glaucoma detection


%In order to summarize the characteristics of the existing databases, we performed a systematic review of the literature to identify those sets. We discarded all those sources that did not include glaucoma classification labels. A summary of the results is provided in Table~\ref{table:database-comparison}. The REFUGE database (Section~\ref{subsec:refuge}) is also included for comparison purposes. %GlaucomaDB \cite{khalil2017improved} was not included because it does not provide glaucoma / non-glaucoma labels but diagnostic opinions from two different experts based on the images and CDR values.


\subsubsection{Number of images and distribution of glaucomatous/non-glaucomatous cases} %Counting with a large number of fundus photographs is essential for developing deep learning based algorithms. So far, the largest database is ORIGA-Light~\footnote{\url{http://imed.nimte.ac.cn/origa-650.html}}, which contains 650 fundus photographs, with approximately 25\% being glaucomatous.\Hc{Is ORIGA publicly available? I thought they took it down for some reason.}

\subsubsection{Ground truth annotations provided with the database} %The availability of multiple labels allows to develop robust algorithms that can leverage the information provided not only by the diagnosis labels but also from other annotations such as segmentations. The data sets DR HAGIS~\footnote{\url{https://www.research.manchester.ac.uk/portal/files/53852982/JMI_4_1_014503.pdf}},  HRF~\footnote{\url{https://www5.cs.fau.de/research/data/fundus-images/}} and LES-AV~\footnote{\url{https://ignaciorlando.github.io/data/LES-AV.zip}} are focused on vessel segmentation and/or artery/vein classification, so no labels for optic disc/cup segmentation are provided. On the other hand, ORIGA-Light contains such segmentations as ellipsoid approximations to the actual morphology. This can affect CDR values when computed using the total area of the structures. Finally, none of these existing data sets provide labels for the localization of the fovea. 
%HRF contains 15 images of glaucomatous patients in advanced stage, 15 with diabetic retinopathy and 15 healthy subjects without any retinal pathology.
% DR HAGIS do not mention

\subsubsection{Images captured with different acquisition devices} %The diversity of devices in the training/validation/test sets is also important to ensure a proper evaluation of the generalization ability of the proposed algorithms. To the best of our knowledge, all the existing databases are focused on 

\subsubsection{Fixed partitions in training/test splits} %are necessary to prevent overfitting and to ensure a proper comparison between different models. All the existing databases contain images captured with the same acquisition device. DRISHTI-GS provides a fixed partition into 50 and 51 images for training and test, respectively. Originally, the test labels were not publicly shared to prevent unfair practices in model selection. Now the labels can be download from the project website, for the full data set.

\subsubsection{Source of the diagnosis provided as ground truth labelling} %The glaucoma labels in DRISHTI-GS1~\cite{sivaswamy2014drishti,sivaswamy2015comprehensive} were assigned by ophthalmologists based on the image appearance.

\subsubsection{Availability of a fixed evaluation framework} %RIM-ONE do not provide a uniform framework for evaluation, although it introduces a metric for comparing different algorithms for optic disc segmentation.

% Some databases contain images of DR or AMD cases (ARIA)
% ARIA~\footnote{\url{https://eyecharity.weebly.com/aria_online.html}} uses low resolution images.
% DRIONS-DB~\footnote{\url{http://www.ia.uned.es/~ejcarmona/DRIONS-DB.html}}
% IDRiD~\footnote{\url{https://idrid.grand-challenge.org}} has images of healthy subjects and patients with DR. Only 81 images have annotations for optic disc segmentation.





\begin{table*}[t]  
\centering
\caption{Comparison of the REFUGE challenge data set with other publicly available data sets.}
\resizebox{\textwidth}{!}{
\begin{tabular}{C{2.64cm}|C{1.25cm} C{1.2cm}|C{0.7cm}| C{1.25cm} C{1cm} C{1.2cm}|C{1.09cm}|C{1.3cm}|C{1.15cm}|C{1.35cm}}
  \hline
  \multirow{2}{2.65cm}{\centering \textbf{Dataset}} & \multicolumn{3}{c|}{\textbf{Num. of images}} & \multicolumn{3}{c|}{\textbf{Ground truth labels}} & \multirow{2}{1.1cm}{\centering \textbf{Different cameras}} & \multirow{2}{1.4cm}{\centering  \textbf{Training \& test split}} & \multirow{2}{1.2cm}{\centering  \textbf{Diagnosis from}} & \multirow{2}{1.4cm}{\centering \textbf{Evaluation framework}} \\
  \cline{2-7}
  & \textbf{Glaucoma} & \textbf{Non glaucoma} & \textbf{Total} & \textbf{Glaucoma detection} & \textbf{Optic disc/cup} & \textbf{Fovea localization} & & & & \\
  \hline
  ARIA~\cite{zheng2012automated} & 0 & 143 & 143 & No & Yes/No & Yes & No & No & ? & No \\
  \hline
  DRIONS-DB~\cite{carmona2008identification} & - & - & 110 & No & Yes/No & No & ? & No & ? & No \\
  \hline
  DRISHTI-GS1 \cite{sivaswamy2014drishti,sivaswamy2015comprehensive} & 70 & 31 & 101 & Yes & Yes/Yes & No & No & Yes & Image & No \\
  \hline
  DR HAGIS~\cite{holm2017dr} & 10 & 29 & 39 & Yes & No/No & No & Yes & No & ? & No \\
  \hline
  IDRiD~\cite{porwal2018indian} & 0 & 516 & 516 & No & Yes/No & Yes & No & Yes & ? & Yes \\
  \hline
  HRF~\cite{odstrcilik2013retinal} & 15 & 30 & 45 & Yes & No/No & No & No & No & Clinical & No \\
  \hline
  LES-AV~\cite{orlando2018towards} & 11 & 11 & 22 & Yes & No/No & No & No & No & Clinical & No \\
  \hline
  ORIGA-Light~\cite{zhang2010origa} & 168 & 482 & 650 & Yes & Yes/Yes & No & ? & No & ? & No \\
  \hline
  RIM-ONE~\cite{fumero2011rim} & 74 & 85 & 169 & Yes & Yes/No & No & No & No & Clinical & No \\
  \hline
  RIGA~\cite{almazroa2018retinal} & - & - & 750 & No & Yes/Yes & No & Yes & No & ? & No \\
  \hline
  \hline
  REFUGE & 120 & 1080 & 1200 & Yes & Yes/Yes & Yes & Yes & Yes & Clinical & Yes \\
  \hline
\end{tabular}}
\label{table:database-comparison} 
\end{table*}

%\textcolor{green}{\cmark}
%\textcolor{red}{\xmark}



